Self-Supervised Attention Learning for Depth and Ego-motion Estimation

We address the problem of depth and ego-motion estimation from image sequences. Recent advances in the domain propose to train a deep learning model for both tasks using image reconstruction in a self-supervised manner. We revise the assumptions and the limitations of the current approaches and propose two improvements to boost the performance of the depth and ego-motion estimation. We first use Lie group properties to enforce the geometric consistency between images in the sequence and their reconstructions. We then propose a mechanism to pay an attention to image regions where the image reconstruction get corrupted. We show how to integrate the attention mechanism in the form of attention gates in the pipeline and use attention coefficients as a mask. We evaluate the new architecture on the KITTI datasets and compare it to the previous techniques. We show that our approach improves the state-of-the-art results for ego-motion estimation and achieve comparable results for depth estimation.

==> architectures/DispNet.tex <==
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Encoder''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
cnv1         & 7               & 2               & 3/32              & 1              & 2               & target                 \\
cnv1b        & 7               & 1               & 32/32             & 2              & 2               & cnv1                \\
cnv2         & 5               & 2               & 32/64             & 2              & 4               & cnv1b               \\
cnv2b        & 5               & 1               & 64/64             & 4              & 4               & cnv2                \\
cnv3         & 3               & 2               & 64/128            & 4              & 8               & cnv2b               \\
cnv3b        & 3               & 1               & 128/128           & 8              & 8               & cnv3                \\
cnv4         & 3               & 2               & 128/256           & 8              & 16              & cnv3b               \\
cnv4b        & 3               & 1               & 256/256           & 16             & 16              & cnv4                \\
cnv5         & 3               & 2               & 256/512           & 16             & 32              & cnv4b               \\
cnv5b        & 3               & 1               & 512/512           & 32             & 32              & cnv5                \\
cnv6         & 3               & 2               & 512/512           & 32             & 64              & cnv5b               \\
cnv6b        & 3               & 1               & 512/512           & 64             & 64              & cnv6                \\
cnv7         & 3               & 2               & 512/512           & 64             & 128             & cnv6b               \\
cnv7b        & 3               & 1               & 512/512           & 128            & 128             & cnv7                \\ \hline
\end{tabular}
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Decoder''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
upcnv7       & 3               & 2               & 512/512           & 128            & 64              & cnv7b               \\
icnv7        & 3               & 1               & 1024/512          & 64             & 64              & upcnv7+cnv6b        \\
upcnv6       & 3               & 2               & 512/512           & 64             & 32              & icnv7               \\
icnv6        & 3               & 1               & 1024/512          & 32             & 32              & upcnv6+cnv5b        \\
upcnv5       & 3               & 2               & 512/256           & 32             & 16              & icnv6               \\
icnv5        & 3               & 1               & 512/256           & 16             & 16              & upcnv5+cnv4b        \\ \hline
upcnv4       & 3               & 2               & 256/128           & 16             & 8               & icnv5               \\
icnv4        & 3               & 1               & 128/128           & 8              & 8               & upcnv4+cnv3b        \\
disp4        & 3               & 1               & 128/1             & 8              & 8               & icnv4               \\ \hline
upcnv3       & 3               & 2               & 128/64            & 8              & 4               & icnv4               \\
icnv3        & 3               & 1               & 129/64            & 4              & 4               & upcnv3+cnv2b+disp4  \\
disp3        & 3               & 1               & 64/1              & 4              & 4               & icnv3               \\ \hline
upcnv2       & 3               & 2               & 64/32             & 4              & 2               & icnv3               \\
icnv2        & 3               & 1               & 65/32             & 2              & 2               & upcnv2+cnv1b+disp3  \\
disp2        & 3               & 1               & 32/1              & 2              & 2               & icnv2               \\ \hline
upcnv1       & 3               & 2               & 32/16             & 2              & 1               & icnv2               \\
icnv1        & 3               & 1               & 17/16             & 1              & 1               & upcnv1+disp2        \\
disp1        & 3               & 1               & 16/1              & 1              & 1               & icnv1               \\ \hline
\end{tabular} 

==> architectures/PoseNet.tex <==
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Encoder - PoseNet''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
cnv1         & 7               & 2               & 3*(1+S)/16        & 1              & 2               & target+ nearby     \\
cnv2         & 5               & 2               & 16/32             & 2              & 4               & cnv1               \\
cnv3         & 3               & 2               & 32/64             & 4              & 8               & cnv2               \\
cnv4         & 3               & 2               & 64/128            & 8              & 16              & cnv3               \\
cnv5         & 3               & 2               & 128/256           & 16             & 32              & cnv4               \\
cnv6         & 3               & 2               & 256/256           & 32             & 64              & cnv5               \\
cnv7         & 3               & 2               & 256/256           & 64             & 128             & cnv6               \\
pose_pred    & 1               & 1               & 256/S*6           & 128            & 128             & cnv7               \\ \hline
\end{tabular}
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Decode - ExpNet Extension''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
upcnv5               & 4               & 2               & 256/128           & 32             & 16              & conv5            \\
upcnv4               & 4               & 2               & 128/164           & 16             & 8               & upconv5          \\
upcnv3               & 4               & 2               & 64/32             & 8              & 4               & upconv4          \\
upcnv2               & 4               & 2               & 32/16             & 4              & 2               & upconv3          \\
upcnv1               & 4               & 2               & 16/8              & 2              & 1               & upconv2          \\ \hline

predict\_mask4       & 3               & 1               & 128/S             & 8              & 8               & upconv4          \\ 
predict\_mask3       & 3               & 1               & 64/S              & 4              & 4               & upconv3          \\
predict\_mask2       & 3               & 1               & 32/S              & 2              & 2               & upconv2          \\
predict\_mask1       & 3               & 1               & 16/S              & 1              & 1               & upconv1          \\ \hline
\end{tabular} 


==> architectures/U-Net.tex <==
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Encoder''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
cnv1         & 3               & 1               & 3/64              & 1              & 1               & target              \\
cnv1b        & 7               & 1               & 64/64             & 1              & 1               & cnv1                \\
cnv2         & 5               & 1               & 64/128            & 2              & 2               & cnv1b               \\
cnv2b        & 5               & 1               & 128/128           & 2              & 2               & cnv2                \\
cnv3         & 3               & 1               & 128/256           & 4              & 4               & cnv2b               \\
cnv3b        & 3               & 1               & 256/256           & 4              & 4               & cnv3                \\
cnv4         & 3               & 1               & 256/512           & 8              & 8               & cnv3b               \\
cnv4b        & 3               & 1               & 512/512           & 8              & 8               & cnv4                \\
cnv5         & 3               & 1               & 512/1024          & 16             & 16              & cnv4b               \\
cnv5b        & 3               & 1               & 1024/1024         & 16             & 16              & cnv5                \\ \hline
\end{tabular}
\begin{tabular}[t]{|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|l|}{\textbf{``Decoder''}} \\
\hline
\textbf{layer} & \textbf{k} & \textbf{s} & \textbf{chns} & \textbf{in} & \textbf{out} & \textbf{input}       \\ \hline
up5          & 3               & 2               & 512/256           & 16             & 8               & conv5b              \\
att5         & 3               & 1               & 512/256           & 8              & 8               & up5,cnv4b           \\ 
upcnv5       & 3               & 1               & 512/256           & 8              & 8               & att5+up5            \\ \hline

up4          & 3               & 2               & 256/128           & 8              & 4               & conv4b*             \\
att4         & 3               & 1               & 128/128           & 4              & 4               & up4,cnv3b           \\
upcnv4       & 3               & 1               & 128/128           & 4              & 4               & att4+up4            \\ \hline

up3          & 3               & 2               & 128/64            & 4              & 2               & conv3b*             \\
att3         & 3               & 1               & 128/64            & 2              & 2               & up3,cnv2b           \\
upcnv3       & 3               & 1               & 128/64            & 2              & 2               & att3+up3            \\ \hline

up2          & 3               & 2               & 64/32             & 2              & 1               & conv3b*             \\
att2         & 3               & 1               & 64/32             & 1              & 1               & up2,cnv1b           \\
upcnv2       & 3               & 1               & 64/32             & 1              & 1               & att2+up2            \\ \hline

disp4        & 3               & 1               & 512/1             & 8              & 8               & upcnv5              \\
disp3        & 3               & 1               & 256/1             & 4              & 4               & upcnv4              \\
disp2        & 3               & 1               & 128/1             & 2              & 2               & upcnv3              \\
disp1        & 3               & 1               & 64/1              & 1              & 1               & upcnv2              \\ \hline
alpha4       & 3               & 1               & 1/2               & 8              & 8               & att5(alpha)         \\
alpha3       & 3               & 1               & 1/2               & 4              & 4               & att4(alpha)         \\
alpha2       & 3               & 1               & 1/2               & 2              & 2               & att3(alpha)         \\
alpha1       & 3               & 1               & 1/2               & 1              & 1               & att2(alpha)         \\ \hline
\end{tabular}

==> chapters/2_problem_statement.tex <==

\chapter{Problem Definition}
In this chapter we provide a detailed definition of depth and ego-motion estimation (also called relative camera pose estimation, we will use these terms interchangeably).
%in a mathematical point of view.

\section{Monocular Depth estimation}
Given an input image from a single (monocular) camera, we want to train a model that is able to estimate, at inference time, the depth for every pixel in the image. Given this formulation, we will have an estimated depth map having the same width and height as the input image, it would corresponds to an additional, depth channel for the image, as shown in Figure\ref{fig:depth}. We need a function $f_d$ that maps every pixel $I_p$ in an RGB image to a depth value $d_p$. Equation~\ref{eq:depth} gives it in a general form, where $I$ is the image and $D$ is the depth:

\begin{equation}
    D = f_d(I),
\label{eq:depth}
\end{equation}
\nointend
where $f_d$ could be any function that takes as input each pixel and estimates its depth individually or uses a patch of the image to estimate the corresponding area depth or processes the whole image. In deep learning, $f_d$ is usually a deep regressor (convolutional neural network, fully connected network, etc.) that takes the whole image as an input and maps directly to the depth map.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/diagram-1.png}
  \caption{Generic view of the regression function mapping an image of width $W$ and height $H$ to a depth map.}
  \label{fig:depth}
\end{figure}

\section{Ego-motion estimation (relative camera pose)}
Given a sequence of $k$ input images taken by a camera (with the same camera intrinsics), we want to estimate, at inference time, the relative camera pose between a target frame $I_t$ and the nearby $k-1$ frames. The relative pose $P$ is represented in the form of the six degrees of freedom (6DoF), $P \in SE(3)$, with three values referring to translation $T=(x, y, z)\in \mathrm{R}^3$ and other three values referring to the rotation $R=$(pitch, roll, yaw), $R \in SO(3)$. Each relative pose represents a transformation from the target image $I_t$ to the corresponding nearby image $I_s$, $s={t-k/2},\ldots,{t-1},t+1,\ldots,{t+k/2}$. Therefore, we can formulate the problem as a function $f_p$ that takes as input $k$ frames and output $k-1$ relative poses, where $P_s$ corresponds to the pose (6-DoF) from $I_t$ to $I_s$. This could be expressed by the following equation:

\begin{equation}
    P = f_p(I_{t - k/2},...,I_{t},...,I_{t+k/2} )
\label{eq:depth}
\end{equation}
\noinednt
where $f_p$ is a function that takes as input a $k$ frames and produces $k-1$ relative poses. In deep learning, $f$ is usually a deep regressor that inputs the concatenated frames and outputs a matrix $P$ of size $(k-1)x6$ as shown in Figure \ref{fig:poses}.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/diagram-2.png}
  \caption{Generic view of the regression function that estimate the relative poses between sequences of $k$ frames.}
  \label{fig:poses}
\end{figure}

While the depth and pose estimations problems are presented separately, they are closely related. Moreover in the next section we will show that the depth estimation function $f_d$ and camera pose estimation function $f_p$ can be coupled in a joint learning procedure able to make two estimations at the same time.

% \textcolor{red}{Definitions are partial and of a high level... Gives no sufficient details on the task complexity and mathematical properties. Do you use these functions $f$ later? Simple space filler. If not extended, this section is better be moved to the beginning of the technical sections.}

% \textcolor{red}{Where are you unifying visual odometry, ego-motion and camera pose estimation ?} 

==> chapters/4_our_works.tex <==
\chapter{Contributions and new approaches}
In this chapter, we consider the task of depth and ego-motion estimation in details. We build on the most polular state of the art baseline approach. We first explain how the baseline architecture solves the problem. We then run a series of ablation studies to discover the strong and potentially weak aspects of the baseline architecture which can be potentially improved. Then we present three proposals to improve the baseline architecture, they represent the main contribution of this work. 

All the implementations were done using PyTorch framework, detailed the neural network architectures will be provided in the appendix.

\section{The baseline architecture}
As the baseline, we consider the seminal work of Zhou et al.~\cite{zhou2017unsupervised}. This work was first to estimate the depth and relative camera pose simultaneously, using a sequence of videos in a fully self-supervised manner. At training time (see figure \ref{fig:Zhou-1}), the framework processes unlabelled video sequences to train both the depth estimation model and the pose estimation model. Once the models are trained, at test time, the inference of the depth and the pose can be done dis-jointly, as each model could be used separately. \\

The signal of self-supervison in the baseline architecture is inspired by the principle of view synthesis \cite{Zhou2016ViewFlow}. Given an input image representing a scene from one point of view, the goal is to synthesize an image looking at the scene from a different point of view. When applying the synthesis principle to the image sequences, we have a target frame and we try to reconstruct (synthesize) it by using the nearby frames. The original architecture is named {\it SfMLearner}, standing for Structure from Motion Learner. It tries to reconstruct the image using a sequence of images which represent a motion.  \\

The baseline architecture includes the depth and pose networks.
During the training phase, the depth network takes the target image and generates the disparity map of the image (in the literature it is sometimes referred as DispNet instead of DepthNet). The disparity values are inversely proportional to the depth values; the generation is done by an encoder-decoder network (see figure \ref{fig:Zhou-2}). Thus, the depth network is a deep dense regressor, it outputs disparity/depth values $\hat{D}_t(p)$ for all pixels in an image, and $p$ indexes over the pixel coordinates. \\

While the depth network processes images individually, the pose network copes with sequence of images. At each step, it concatenates the target image and two nearby images (e.g. $I_{t-1}$ and $I_{t+1}$) over the RGB channels in a specific order (the target image $I_{t}$ first, then the previous image $I_{t-1}$, then the following image $I_{t+1}$).  The new concatenated tensor is fed to the pose network (PoseNet), the network outputs the relative camera poses ($\hat{T}_{t\rightarrow t-1}$, $\hat{T}_{t\rightarrow t+1}$). The network is a dense deep network that regresses the six degree of freedom values (three for translation $Tr$=($x,y,z$) and three for rotation $R$=(pitch, yaw, roll) per nearby image, and these values are then used to reconstruct the transformation matrix $T=(Tr,R)$. \\

%INVERSE WARPING OPERATION
We use a known technique from computational photography, called {\it inverse warping}. This technique is differentiable, thus it allows to back-propagate the gradients to the networks while training. The idea is simply to reconstruct the target image $I_{t}$ by sampling pixels from the two neighbour images (e.g. $I_{t-1}$ and $I_{t+1}$) based on the estimated depth map $\hat{D}_t$ and the relative transformation matrices ($\hat{T}_{t\rightarrow t-1}$, $\hat{T}_{t\rightarrow t+1}$), as shown in figure \ref{fig:inverse_warping}. The sampling is done by using the transformation equation \ref{eq:inverse_warping} that maps the homogeneous coordinates of the target pixel $p_t$ to the projected coordinate onto the source pixel $p_s$. As we see in the equation we need to know the camera intrinsics $K$, the estimated depth of the pixel $\hat{D}_t(p)$ and the transformation matrix between the two images $\hat{T}_{t\rightarrow s}$:

\begin{equation}
    p_s \sim K \hat{T}_{t\rightarrow s}\hat{D}_{t}(p_t)K^{-1}p_t
    \label{eq:inverse_warping}
\end{equation}

When we project the target pixel $p_t$ to the nearby pixel $p_s$ we get a continuous values for the coordinates (see figure \ref{fig:inverse_warping} b) which do not represent any pixel in the nearby image. We then use the differentiable bi-linear sampling interpolation introduced in the \textit{Spatial Transformer Networks} \cite{Jaderberg2015SpatialNetworks}. We interpolate the value of RGB for the projected pixel using the 4-pixel neighbours at the corners of $p_s$ (top-right, top-left, bottom-right, bottom-left) to get the values of $p_t$ in the new reconstructed image $\hat{I_s}$. The interpolation is done using this equation \ref{eq:interpolate}, where  $\hat{I}_s(p_t)$ is the final RGB values at position $p_t$ in the reconstructed image $\hat{I_s}$, $I_s(p_s)$ is the unknown RGB of the continuous coordinate in the nearby frame and the $w^{ij}$ is linearly proportional to the spatial proximity between $p_s$ and the corner pixel $p_s^{ij}$. Normally, $w^{ij} = 0.25$ and sum to 1.


\begin{equation}
    \hat{I}_s(p_t) = I_s(p_s) = \sum_{i\in\{t,b\}, j\in\{l,r\}}w^{ij}I_s(p_s^{ij})
    \label{eq:interpolate}
\end{equation}


At the end, when we get the reconstructed images by the set $\textbf{S}$ of N nearby images, we can apply a similarity loss between every reconstruct target image $\hat{I}_{k}(k \neq t)$ and the real target image $I_{t}$. In the baseline, they used the L1 loss objective function (i.e., the photometric/photo-consistency loss) as follow:
\begin{equation}
    \mathcal{L}_{p} = \sum_{<I_1, \ldots, I_N> \in \textbf{S}}\sum_p  | I_t (p) - \hat{I}_s(p) |~.
\label{eq:photo}
\end{equation}

Till now, the model faces some limitations as the author confirms in his work. The view synthesis module assumes that the scene has rigid objects with no occlusion between the target view and nearby views and that the surface is Lambertian, so we can apply the photometric loss \ref{eq:photo} directly as described above. But in reality, these assumptions are violated between some training examples which affect drastically the training procedure. To overcome these limitations, the author introduces a new module under the name of \textit{explainability}. the aim of the module is to indicate the importance of each pixel, if it should be considered during the view synthesis faces or not. If the pixel will contribute to a corrupted synthesis (because of the  violation of the cited assumptions), the explainability value of the pixel will be negligible. \\

\begin{figure}[H]
\centering
  \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{pics/relative_pose.png}
    \caption{The relative transformation between two different views for the same camera}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\linewidth}
    \includegraphics[width=\linewidth]{pics/Zhou-3.png}
    \caption{The sampling step and interpolation step}
  \end{subfigure}
  \caption{Illustration to show how inverse warping is used to reconstruct a target image}
  \label{fig:inverse_warping}
\end{figure}




This new module is trained jointly and simultaneously with the depth and pose modules (figure \ref{fig:Zhou-2}.  It is an encoder-decoder architecture as well. PoseNet acts as the encoder part of the explainability network, except the last layer that generate $N$ 6-DoF that does not contribute to the explainability. The decoder generates a per pixel mask $\hat{E}_k(p)$. Similar to PoseNet, the mask map $\hat{E}_k$ (explainability map) is generated for both neighbour images, thus, we have $N$ maps generated by the new network. 

Using this new output, we will embed it in the photometric loss \ref{eq:photo} to get:

\begin{equation}
    \mathcal{L}_{p} = \sum_{<I_1, \ldots, I_N> \in \textbf{S}}\sum_p \hat{E}_k(p) | I_t (p) - \hat{I}_s(p) |~.
\label{eq:exp}
\end{equation}

% \begin{equation}
%   \mathcal{L}_{reg}(\hat{E}_k^l) = | \hat{E}_k^l - 1 |~.
% \label{eq:exp}
% \end{equation}

If we train the network with the modified loss \ref{eq:exp}, we get a trivial solution with $\hat{E}_k(p)$ equals to zero, which reduces the loss to zero. To overcome the optimization problem, we have to put a constraint on the values of $\hat{E}_k(p)$. The constraint could be implemented by adding a regularization loss  $\mathcal{L}_{reg}(\hat{E}_k)$. This is a cross entropy loss between the mask value and a constant label 1 that encourages a non-zero predictions in this case. \\

% WRITE DOWN THE EXPLAINABILITY REGULARIZATION LOSS
% \begin{equation}
%     \mathcal{L}_{p} = \sum_{<I_1, \ldots, I_N> \in \textbf{S}}\sum_p \hat{E}_k(p) | I_t (p) - \hat{I}_s(p) |~.
% \label{eq:exp}
% \end{equation}

%WRITE ABOUT THE DEPTH SMOOTH LOSS
As the depth discontinuities often occur at image gradients, we penalize the L1 norm of the second gradients of the depth map. As a result, we get not constant but rather smoothly changing depth values. The loss is adapted from \cite{Vijayanarasimhan2017SfM-Net:Video} describe as below:

\begin{equation}
    \mathcal{L}_{smooth} = | \nabla_{xx} D | +| \nabla_{yy} D |+ | \nabla_{yx} D |+ | \nabla_{xy} D |~.
\label{eq:smooth}
\end{equation}

\begin{equation}
\mathcal{L}_{smooth} = \sum_p|\nabla D(p)|^{T} \cdot e^{-|\nabla I(p)|} 
\label{eq:smooth}
\end{equation}

Thus, the full training loss will be:

\begin{equation}
    \mathcal{L}_{final} = \sum_l \mathcal{L}_{p}^l +  \lambda_{smooth} \mathcal{L}^l_{smooth} + \lambda_{reg} \sum_{s} \mathcal{L}_{reg}(\hat{E}_k^l)~,
\label{eq:full}
\end{equation}

The $\lambda_{smooth}$ and $\lambda_{reg}$ are hyper-parameters. We sit them to 0.1 which gave us the most stable results.

We did not apply only the loss over the last output. As mentioned in figure \ref{fig:Zhou-2} we applied on three additional intermediate layers from DepthNet and ExpNet. For this reason in the final loss equation \ref{eq:full} we sum over the layers indexed by $l$.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/Zhou-1.png}
  \caption{A general overview of SfMLearner \cite{Zhou2017Unsupervised} in Training Time }
  \label{fig:Zhou-1}
\end{figure}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/Zhou-2.png}
  \caption{The architecture of Depth (on the left) and Pose/Explainability (on the right) models}
  \label{fig:Zhou-2}
\end{figure}

\begin{figure}[H]
\centering
  \includegraphics[scale=0.5]{pics/teaser.pdf}
  \caption{A general overview of SfMLearner \cite{Zhou2017Unsupervised} in Test time}
  \label{fig:Zhou-teaser}
\end{figure}

\section{Approach 1: GAN-based architecture (Adversarial approach)}
% \lipsum[1-3]

%WRITE ABOUT GAN AND THE MOTIVATION
With the rise of Generative Adversarial Networks (GANs) \cite{Goodfellow2014GenerativeNetworks} in various applications \cite{Isola2017Pix2pix,Zhu2017UnpairedNetworks,Pilzer2018UnsupervisedNetworks,Atapour-Abarghouei2018Real-TimeTransfer}, we started an hypothesis that is based on the adversarial training introduced in \cite{Goodfellow2014GenerativeNetworks}. We have noticed that we can take benefits from the N reconstructed images: We know that these images are "Fake" images, and the only corresponding real image is the target image. Thus, as shown in Figure \ref{fig:GAN}, instead of only applying the photometric loss \ref{eq:photo} between the synthesized images and the target image, we can feed the synthesized images to a discriminator labeled as "Fake" images. The target image will be fed as well to the discriminator labeled as "Real" image. Then, if we treat the whole baseline (DepthNet + PoseNet) as a "Generator", we can apply the adversarial loss equation \ref{eq:GAN_cross_entropy} between the generator and the discriminator as shown below, where $\textbf{R}$ and $\textbf{F}$ correspond to the set of real and fake images, respectively. $D$ and $P$ are the depth and the poses respectively.

\begin{equation}
\min_G \max_D V(D, G) = \mathbb{E}_{\bm{r} \sim \textbf{R}}[\log D(\bm{r})] + \mathbb{E}_{\bm{f} \sim \textbf{F}}[\log (1 - f)], where \quad f = G(D,P).
\label{eq:GAN_cross_entropy}
\end{equation}

The figure \ref{fig:GAN} illustrate an abstract view of the new architecture. We will elaborate the different discriminators and adversarial losses we used to get a stable training phase.\\

%DIFFERENCE FORM OF DISCRIMINATORs (DCGAN = ImageGAN, PatchGAN, PixelGAN)
We started by the discriminator architecture introduced in \cite{Radford2015UnsupervisedNetworks}, which is referred to DCGAN. The discriminator is an encoder architecture which takes as input the whole image and keeps down-sampling the input using the strided convolution operation until it outputs a single value that corresponds to the probability of the image to be real. Like \cite{Zhu2017UnpairedNetworks}, we refer to this architecture as ImageGAN, since the discriminator receptive field is the whole image. \\ 

A second alternative, the PatchGAN, used in the recent style and texture transfer techniques \cite{Li2016PrecomputedNetworks,Isola2017Pix2pix,Zhu2017UnpairedNetworks,Ledig2016Photo-RealisticNetwork} was implemented and tested. Unlike ImageGAN, the discriminator outputs a probability map instead of a single value probability. each value in the map gives the probability that a corresponding patch in the image is real or fake. Thus, in this case, the receptive field is not the whole image, but a patch from the image. This is mathematically equivalent to divide the image into overlapped patches and feed every patch separately to the discriminator that outputs a single belief value like ImageGAN but for every patch, and then average all outputs to get one single probability for the image. We have implemented a PatchGAN that corresponds to 70x70 receptive field.\\

The last alternative is PixelGAN. This architecture is simply a PatchGAN but with a receptive field 1x1. It will correspond, in the end, to a probability map of the same size of the input image that gives for every pixel in the image the probability of being real or fake. The configuration can be implemented using a series of 1x1 convolution that change the dimensionality of the pixels features. Usually, PixelGAN is not used as the best option in the recent style transfer problems because it gives blurry images at the end of training the generator. In our case, it was the best in term of numerical results, which we will elaborate on the results section.\\

%WRITE ABOUT THE DIFFERENT GAN Losses
Despite the adversarial cross entropy loss \ref{eq:GAN_cross_entropy}, we have also tried the mean square error loss (squared L2 norm) \ref{eq:GAN_mse}

\begin{equation}
\min_G \max_D V(D, G) = \mathbb{E}_{\bm{r} \sim \textbf{R}}[ \left( D(\bm{r}) \right)^2] + \mathbb{E}_{\bm{f} \sim \textbf{F}}[\left( 1 - f \right)^2 ], where \quad f = G(D,P).
\label{eq:GAN_mse}
\end{equation}

Thus the final loss $\mathcal{L}_{final GAN}$ will have an extra hyper-parameter $\lambda_{GAN}$ which we found to be 0.5. As shown in equation \ref{eq:gan_full}, the summation over the fake images is mentioned, because normally in GAN we have one fake image for every real image, but in our case, we have N generated fake images, thus we feed them all to the discriminator. 

\begin{equation}
    \mathcal{L}_{final GAN} = \sum_l (\mathcal{L}_{p}^l +  \lambda_{smooth} \mathcal{L}^l_{smooth} + \lambda_{reg} \sum_{s} \mathcal{L}_{reg}(\hat{E}_k^l)) + \lambda_{GAN} \sum_{f} \mathcal{L}_{GAN}(f)~,
\label{eq:gan_full}
\end{equation}

%HOW TO SLOW DOWN DISCRIMINATOR
In GANs, the discriminator and generator are updated at each iteration. In this setting,We found that the discriminator has more advantage to beat the generator after the first training epoch, and it affects drastically the performance of the generator. We have to avoid this problem by slowing down the discriminator training, and update it only once every 10 updates of the generator. This problem was crucial because it is very easy for the discriminator to distinguish the fake images because as we see the inverse warping is not always successful at the beginning.  We can see this problem in the vertical thin shape (like the sign on the road) that are broken in the reconstructed images in figure \ref{fig:gan_failure_results}.

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/diagram-4.png}
  \caption{Proposed GAN model}
  \label{fig:GAN}
\end{figure}


\section{Approach 2: Backward-Forward Consistency Loss (Geometry-based approach)}
% \lipsum[1-3]
%MOTIVATION
Another aspect is tackled: The geometric aspect between camera poses. We know that any transformation in 6DoF has a reverse transformation. From mathematical point of view, every 4x4 transformation matrix has an inverse. From this simple idea, we started another approach to put an additional consistency next to the photometric consistency. \\

Since we have PoseNet that regress the pose from the target frame to the nearby frame, we can also generate the inverse pose (from the nearby frame to target frame). For example, we will have at the end the original transformation $\hat{T}_{t\rightarrow t-1}$ and the inverse  $\hat{T}_{t-1\rightarrow t}$ \\


As shown in figure \ref{fig:BF}, using 5 sequential frames, we can concatenate the frames differently for the seek of having the inverse transformations. This means treat every nearby frame with the same manner as the target frame to get 6DoF from the nearby frame to the target frame which means the inverse of original transformation. In this case we will get 2 couples of transformations matrices: $(\hat{T}_{t\rightarrow t-1}$,$\hat{T}_{t-1\rightarrow t})$  and $(\hat{T}_{t\rightarrow t+1}$,$\hat{T}_{t+1\rightarrow t})$.\\

%EXPLAIN THE LOSS
Using every couple of transformation $\hat{T}_{t_1\rightarrow t_2}$ and $\hat{T}_{t_2\rightarrow t_1}$, we can apply an additional similarity loss. Since the multiplication of a matrix by its inverse should be identity, we will apply a norm loss in equation \ref{eq:BF} between the multiplication and the identity matrix $I_{4x4}$ as shown below, where \textbf{T} is all the couples of transformation matrices we can get, indexed by q:

\begin{equation}
    \mathcal{L}_{BF} = \sum_{q \in \textbf{T}}| \hat{T}^q_{t_1\rightarrow t_2}\hat{T}^q_{t_2\rightarrow t_1} - I_{4x4} |~.
\label{eq:BF}
\end{equation}


\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/diagram-3.png}
  \caption{Proposed model with Backward-Forward Consistency loss}
  \label{fig:BF}
\end{figure}

%PROOF OF ITS EFFECTIVENESS
To proof the effectiveness of this loss, we added it the baseline final loss in equation \ref{eq:full} and give it a higher importance comparing to other losses. This is done by adding a weighting parameter $\lambda_{BF}$ and give it a very high value equals to 100, which means 100 bigger than the original photometric loss. Thus, the neural networks updates are more biased to minimize this loss. As shown in figure \ref{fig:BF_proof}, a trajectory for the camera poses equivalent to straight line is generated instead of the ground truth trajectory, because it is very easy for the network to have optimize in one direction of the 6DoF with minimum rotation that guarantees a consistency with the inverse matrix.

\begin{figure}[H]
\centering
  \includegraphics[scale=0.35]{pics/BF-effective.png}
  \caption{Generated camera poses trajectory with high bias to minimize the Backward-Forward consistency loss}
  \label{fig:BF_proof}
\end{figure}

\section{Approach 3: Introduce Attention modules (Visual-based approach)}
% \lipsum[1-3]
%MOTIVATION (DEPTH ESTIMATION AS IMAGE SEGMENTATION)
Despite the geometric information, the last approach focus on the visual information. It is inspired by the works done in semantic segmentation applied in medical imaging tasks \cite{Oktay2018AttentionPancreas, Schlemper2018Attention-GatedDetection}. In these works, they introduce what we call "Attention Modules". As we can see in figure \ref{fig:Attention1}, the attention gate are added in the U-Net shape architecture (similar to DispNet/DepthNet) to extract information jointly from coarser feature map (the gate $g$) and the current high level feature map (the input $x^l$) to know which pixels we have to pay more attention. This is translated in the form of attention coefficients per pixel, $\alpha(p) \in [0,1]$ (see the equations below) that identify the salient image regions that we can see in figure \ref{fig:attention_results}. This technique helps to suppress feature responses in irrelevant background regions.

\begin{gather}
q^l_{att} = \psi^T \left(\, \sigma_1\,(\,W_x^T x_i^l + W_g^T g_i + b_g\,)\,\right) + b_{\psi} \\
\alpha_i^l = \sigma_2 (\, q^l_{att}(x_{i}^l\,,\, g_i \,;\, \Theta_{att}) \,),
\end{gather}

We want to treat depth estimation as semantic segmentation problem. If we consider that each instance (group of pixels) belong to a certain label (e.g. pedestrian, car, road sign), the same group of pixels will have normally the same depth estimated all over the region. Thus, we implemented the attention module inside the DispNet architecture and also we tried the classical Attention U-Net introduced in \cite{Oktay2018AttentionPancreas, Schlemper2018Attention-GatedDetection}. As shown in figure \ref{fig:Attention1}, that during decoding, we don't concatenate the finer layer as it is. We take, instead, the output of the attention gate $\hat{x^l}$ which is the element-wise multiplication of finer feature map $x^l$ and the attention coefficients: $\hat{x^l} = x^l.\alpha$. \\


\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/attention/figure4.pdf}
  \caption{U-Net with the integration of Attention modules}
  \label{fig:Attention1}
\end{figure}

In addition to integrating attention modules to the depth net, we want to take benefit of the attention coefficients $\alpha$ as masking coefficients instead of explainability masks. Thus we modify the photometric loss function to be as in equation \ref{eq:attention_mask}. We then observe how it will change in the behaviour of the coefficients at the end of the training (figure \ref{fig:attention_results}.

\begin{equation}
    \mathcal{L}_{p} = \sum_{<I_1, \ldots, I_N> \in \textbf{S}}\sum_p \alpha(p) | I_t (p) - \hat{I}_s(p) |~.
\label{eq:attention_mask}
\end{equation}

\begin{figure}[H]
  \includegraphics[width=\linewidth]{pics/attention/figure3.pdf}
  \caption{Attention module from inside}
  \label{fig:Attention2}
\end{figure}


% \section{Approach 4: Introduce sequential learning}
% \lipsum[1-3]


==> chapters/6_Conclusion.tex <==
\chapter{Conclusion}

We have presented three extensions of the baseline architecture for the depth and pose estimation tasks, all aimed to improve the performance in the self-supervised setting. Now we draw some conclusions from the evaluation results reported in the previous chapter.

\begin{itemize}
\item We have seen that adding backward-forward consistency loss to the training process allowed to boost the performance. Our method follows one of the current trend of combining the deep learning and 3D geometry. It consists in forcing the learned models to respect the geometric principles but adding penalties for any consistency violation. 
This idea opens a possibility to explore and impose more geometric constraints on the learned models, this might further improve the accuracy. There are a number of geometric properties of visual scenes described in the 3D vision literature; we are looking for exploring some of them in the future. 

\item Trying adversarial learning on the depth and pose estimation tasks does not come to a simple conclusion. Evaluation results show how difficult is to maintain the stable and consistent training and inference; this is particularly true for depth estimation. It raises the issue of looking for alternative solutions for the image reconstruction step, which is currently totally based on the inverse warping. One of possible solutions might be in using Bundle Adjustment to fine-tune the image reconstruction module and to force the generator to better estimate the depth and pose.

\item So far, attention models have been successful in Natural Language Processing and some computer vision tasks, such as image classification and semantic segmentation. We explored the usability and effectiveness of attention modules for U-Net architecture for the depth estimation. It shows that attentions principle can be expanded to navigation and localization tasks. In addition, the attention model can be explored as masking coefficients in multiple different ways, it represents a strong alternative to the explainability network in the baseline architecture. 
\end{itemize}

Beyond the three extensions presented above, in the future work, we would like to extend the model with a ConvLSTM component. By training the deep networks with non-annotated videos, it appears natural to take benefit from the temporal relationship between frames in a sequence. We believe that adding a ConvLSTM can boost the performance of pose estimation. Moreover, the depth network in the current configuration obtains information about the relationship between frames indirectly through the photometric loss; so we believe that it should get direct information about the relationship between the frames. This raises the issue of a closer integration of the pose and depth networks. Instead of keeping the two networks decoupled as implemented in the baseline and its variations, sharing some hidden layers can help propagate faster information about the relationships between frames.

==> iros/introduction-1.tex <==
\section{INTRODUCTION}
\label{sec:intro}

The tasks of depth estimation and visual odometry are longstanding problems in computer vision; their successful solution is crucial for a wide variety of applications, such as autonomous driving, robot navigation and visual localization, Augmented/Virtual Reality (AR/VR) applications, etc. {\it Depth estimation} is the process of estimating the relative position between an object (camera, robot, car) and the objects in front of him
%, or even for all surrounding objects in case of a 360 field of view. 
{\it Visual odometry} (VO) is the process of estimating the ego-motion of a camera from a sequence of images. Being one of the most essential technique for camera pose estimation and robot localization, it has attracted a significant interest in both computer vision and robotics communities~\cite{all}.  %It provides similar information for the robot like the GPS and Navigation devices. 

% geometry wang17 (TO BE REVIEWED)
%Since 1990s, considerable works have been accomplished to develop an accurate and robust visual odometry system. As shown in figure~\ref{fig:pipeline} (see chapter 3), a classic pipeline typically consists of a number of critical components, including camera calibration, feature detection, feature matching (or tracking), outlier rejection (e.g., RANSAC), motion estimation, scale estimation and local optimization (Bundle Adjustment). These components have been developed and the entire pipeline has been broadly accepted as a rule of thumbs to follow. Although some state-of-the-art algorithms based on this pipeline have shown excellent performance in terms of accuracy and robustness, they are usually hard-coded with significant engineering effort and each module in the pipeline needs to be carefully designed and fine-tuned to ensure the performance. 

%wang17 %[wang19]
%Nowadays, Deep Learning (DL) dominates various computer vision tasks, with very promising results in image classification \cite{KrizhevskyImageNetNetworks}, object recognition \cite{Girshick20142014RCNN} and semantic segmentation \cite{Li2017FullySegmentation}. Most of the existing deep learning architectures are essentially designed to tackle these classical computer vision problems.
%, with other tasks taking a benefit of pre-trained Convolutional Neural Network (CNN) models to extract high-level representation from images; in such a case CNNs are used as {\it feature extractors}. 
In the last years, 
%the CNNs have been extended to other domains including the visual odometry, depth estimation and 3D geometry. Recently, 
deep learning networks~\cite{Liu2016LearningFields,eigen2015predicting,Garg2016UnsupervisedRescue,zhou2017unsupervised} have started to compete with traditional geometric methods for depth estimation in measurable areas; they achieve competing results in complex and ambiguous 3D areas, with CNNs serving as {\it deep regressors} and often conpounded with more classical components. For the ego-motion estimation, several works \cite{zhou2017unsupervised,Kendall2015PoseNet:Relocalization} have achieved a level of performance comparable to the traditional techniques based on SLAM algorithm \cite{Gomez2018VisualCase,Mur-Artal2015ORB-SLAM:System,Mur-Artal2017ORB-SLAM2:Cameras}. 

%Monocular depth estimation, mahjourian18
Early methods were based on supervised learning for depth and ego-motion, they require large annotated datasets and calibrated setups. 
Often trained and tested one publicly available benchmark datasets
%like Cityscapes, NYU and KITTI, 
these supervised learning techniques show a limited capacity to generalize beyond the data they are trained on. 
%Moreover, available depth ground-truth depth data are often sparse and imperfect, thus causing a range of distinct prediction artifacts. Actually, during the data collection phase, a synchronization between LIDAR sensors and camera is required. 
%Meanwhile, in practice, the rotation of LIDAR scanners sometimes fail to produce a perfect depth data aligned with the pixels of image taken by a camera. 
%The same mismatch problem is even more frequent in camera pose data, where annotations come from GPS and speed sensors, making these annotations noisy and inaccurate. 

%---- (TO BE EDITED) ---------
In addition, while annotating depth data, the annotations suffer from the structural artifacts, particularly in presence of reflective, transparent, dark surfaces or non-reflective sensors which output infinity values. There is usually a shift between the depth sensor and the camera, which causes gaps or overlaps when the point cloud is projected onto the camera's viewpoint. These problems lead to artifacts in models trained on such a noisy data. All these challenges strongly motivated the shift to the unsupervised learning of depth and ego-motion from monocular (single-camera) videos. Using the monocular setting aims to minimize the dependency of stereo camera. %Indeed, in case of failure of one of the cameras, the robot can still learn and act. 

In this work, we address the problem of 3D geometry and ego-motion understanding without annotated training data. The only form of supervision in such a setting is {\it self-supervision}; it instead makes an assumption of consistency and temporal coherence between consecutive frames in a monocular video. The only external data we need is the camera intrinsics. A very recent progress in the domain allows us to use only unlabeled videos to provide self-supervision signals to a learning component. The 3D geometry estimation includes per-pixel depth estimation from a single image and the motion understanding includes camera motion (6DoF relative pose estimation). 

%======================================================
%\subsection{New Extension to Attention etc.}

%TO DO: Starting with Zhou as baseline, discuss previous improvements cite/explain recent improvements, including GANVO, nips19, icra19.

Rigid transformations due to the obstacles, moving objects and reflection effects, where the warping-based image reconstruction is penalised by photo effect of like reflection etc.

Raise issues : extra-cost, buts still a gap with respect to the supervised learning 

Multiple improvements have been proposed to address these issues~\cite{almalioglu2018ganvo, wang19icra,nips19,iros18} are often based on adding more components to the architecture like flow nets~\cite{}, COI ~\cite{graph match}, adversarial networks~\cite{almalioglu2018ganvo}, etc.. These approaches
lead however to excessive and redundant use of computational resources and an important growth of model parameters, make the overall training procedures more complex.  

To address this general problem, we propose a simple and yet effective solution, namely attention gates (AGs). Deep models with AGs can be trained from scratch in a standard
way and AGs automatically learn to focus on image structures without additional supervision.
At test time, these gates generate soft region proposals implicitly on-the-fly and highlight salient features useful for a specific task. Moreover, they do not introduce significant
computational overhead and do not require a large number of model parameters. In return, the proposed AGs improve model sensitivity and accuracy for dense depth predictions
by suppressing feature activations in irrelevant zones. 
In this way, the necessity of using an external organ
localisation model can be eliminated while maintaining the
high prediction accuracy.

%------------------- Contribution -----
We contribute to both geometric and visual components of the training self-supervised DEM estimation models. 

? Self-attention as a strong alternative 
Alternative self-attention as alternative to masking 
and segmentation mechanisms, integration both geometric and visual components

%We first revise the geometric components of the system, in particular, in the reconstrution loss, consistency constraints, intensively used in the state of art. 
We first reinforce the loss by adding an additional constraint, when backward and forward pose transformations should satisfy the Lie group features.
%an inverse should satisfy the Lie group properties. 
Expressed in the form of additional loss term, we integrate it in the consistency loss.  

Then we revise the visual component of the system and 
the reconstruction loss should be weighted differently

%Masking, whihc amchensim to detecet the mor
%exclude thse zoen. We is a weighed
%Inverse , small weights

We propose a self-attention masking to the irrelevant zone of the images. 
Attention mechanism is an alternative to the previous mask mechanisms.
Current solutions add additional loss or components. We show that attention gates can be naturally integrated into the depth network and require no additional components and and a minimal overhead for the training time.

Initially proposed for natural language processing task~\cite{}, the attention mechanism has been successfully extended to vision tasks, including semantic segmentation, cite more here (?)
and a close task of recently for the depth estimation ~\cite{wang2019depth_attention}.
In the case of depth estimation, attention mechanism allows to pay attention to 
Inspired by these recent success we integrate the attention mechanism in the depth and and ego motion unsupervised learning. 

%We denote depth and ego-motion (DEM) unsupervised learning  

%We pursuing the same goal, but we propose different solution, based on the Attention U-net allowing to integrate the weighting coefficients in the . 
Consequently, the depth network can predict both the depth estimation 
and attention mask which is then used to weigh the difference between the true and reconstructed pixels in the total loss. 

%To our best knowledge, this a first attempt to integrate the forward-backward consistency the and attention module in the learning process.  

%Examples in Section~\ref{sec:eval} demonstrate the effect of self-attention on the weighting down and correcting the depth and pose values.


% ---------- Proposal ------------
%In the following sections, we first revise the state of the art techniques for the monocular depth and pose estimation. Then we study a number of modifications aimed to further improve the accuracy at both tasks. 
The main contributions of this work are as follows:
\begin{enumerate}
%\item We propose a new implementation of the baseline architecture for depth and pose estimation~\cite{zhou2017unsupervised}; we revise and improve some components, making the code working faster.

%\item We then show the generative adversarial networks ({\it GANs})~\cite{Goodfellow2014GenerativeNetworks} can help in the most critical phase of the baseline architecture: the image reconstruction. Indeed, the essential part of the network is to use depth and pose in order to reconstruct a given (target) image in a sequence from neighbour images and to compare the reconstruction to the true image. The system learns how to estimate both depth and pose to make the image reconstruction as accurate as possible. Therefore, we imagine a GAN architecture where a discriminator is trained to distinguish between the reconstructed ("fake") images and the real ("true") images. Then, if the whole baseline (DepthNet + PoseNet) is considered as a generator, we can train a discriminator to distinguish between the reconstructed and real images  and to force the generator to synthesize more and more accurate reconstructions, through accurate depth and pose estimation models.
% High quality of reconstruction indicates that depth and pose are estimated correctly.

\item In the computer vision and robotics communities, there exists a clear understanding that pure learning methods fail to grasp the 3D geometry of the visual scenes. Therefore, a new generation of deep models should respect the geometric laws, this represents the most promising research direction in the domain. We adopt this idea and propose a method able to {\it couple geometry with learning} by adding more 3D consistencies in the learning process.

%Extend the existing by backward-Forward constraints.

\item We then introduce {\it attention models} for depth estimation as a new masking technique. Attention models have recently shown very promising results in image classification and segmentation. In a nutshell, an attention model assumes that not all pixels in an image are important for performing a given task, and it learns how to identify the most valuable zones. We show that the attention principle can be extended to the depth estimation as well. We show that an accurate depth estimation of certain zones is more important than others and paying attention to these zones improve the accuracy.
% , we can make the estimated depth maps sharper and more accurate.
%\item We finally report an extended evaluation of all developed methods on KITTI Visual Odometry dataset.
\end{enumerate}

%The remainder of the paper is organized as follow. First, we formally define the problem of depth and pose estimation. Second, we review and analyze the state of the art, paying a particular attention to the very recent works on the self-supervision by means of image reconstruction. Thirdly, we present our baseline architecture in details and describe three implemented extensions aimed to improve the accuracy of both depth and pose estimation. namely, we present the GAN extension, an extension with additional geometric constraints, and an extension with an attention model. Finally, we present the KITTI evaluation test-bed, present results and multiple evaluations, and finally draw some conclusions.

This paper tackles these challenges by proposing a geometry consistency loss for scale-consistent predictions and an induced self-discovered mask for handling moving objects and occlusions. Since we do not leverage multi-task learning like recent works, our framework is much simpler and more efficient. Comprehensive evaluation results demonstrate that our depth estimator achieves the state-of-the-art performance on the KITTI dataset.

The proposed network is trained using unlabeled monocular stereo image pairs and is shown to provide superior performance in depth and ego-motion estimation compared to the existing state-of-the-art.

==> macros.tex <==
\usepackage{times,epsfig,graphicx}
\usepackage{algorithm,algorithmic}
%\usepackage[usenames]{color}
%\usepackage{amssymb,amsmath}
%\usepackage[latin1]{inputenc}
%\usepackage{fancyhdr}
%\usepackage{verbatim}
%\usepackage{tabularx}
%\usepackage{hyperref}
%\usepackage{float}
%\usepackage{bbm}
%\usepackage{dsfont}
%\usepackage{xspace}
%\usepackage{bm}

\newlength{\smallimage}
        \setlength{\smallimage}{0.8cm}
        \setlength\fboxrule{2pt}
        \setlength\fboxsep{0pt}
        \definecolor{rel}{rgb}{.1,.6,.2}
        \definecolor{nrl}{rgb}{1,1,1}
        \definecolor{qim}{rgb}{1,1,1}


%\newcommand{\note}[1]{({\color{green}#1})}
\newcommand{\todo}[1]{({\color{red}ToDo: #1})}
\newcommand{\rk}[1]{{\color{red}{\bf #1}}}
\newcommand{\mk}[1]{{\color{magenta}{\bf #1}}}
\newcommand{\bk}[1]{{\color{blue}{\bf #1}}}
\newcommand{\gk}[1]{{\color{green}#1}}

\makeatletter

\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}


\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot} 
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}


%Specific macros for math symbles
\newcommand{\ka}{k\prime}
\newcommand{\ia}{i\prime}
\newcommand{\logl}{\mathcal{L}}
\newcommand{\deriv}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\minus}{\textrm{-}}
\newcommand{\plus}{\textrm{+}}
\newcommand{\Gauss}[3]{\mathcal{N}(#1;#2,#3)}
%\newcommand{\Gaussd}[2]{\mathcal{N}(#2,#3)}
\newcommand{\T}{\top}
\newcommand{\trans}[1]{#1^{\T}}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\norm}[1]{\parallel\!#1\!\parallel}
\newcommand{\snorm}[1]{\norm{#1}_2^2}
\newcommand{\snormw}[1]{\norm{#1}_W^2}
\newcommand{\ind}[1]{[\![#1]\!]}
\newcommand{\hinge}[1]{[#1]_{+}}
\newcommand{\dotp}[2]{\langle #1,#2 \rangle}
\newcommand{\bigo}[1]{\mathcal{O}(#1)}
\newcommand{\kl}[2]{\mathcal{D}_{\textsc{KL}}(#1||#2)}
\newcommand{\dwd}{d_{W}^{\textrm{dotp}}}
\newcommand{\rank}[1]{\textrm{rnk}(#1)}

\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\rarr}{$\rightarrow$}
\newcommand{\larr}{$\leftarrow$}
\newcommand{\mysec}[1]{section~\ref{#1}}
\newcommand{\fig}[1]{Figure~\ref{#1}}
\newcommand{\tbl}[1]{Table~\ref{#1}}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eqp#1{(\ref{eq:#1})}
\def\eq#1{Eq.~\ref{#1}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ben{\begin{eqnarray*}}
\def\een{\end{eqnarray*}}


\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}

\def\algo#1{Algorithm~\ref{algo:#1}}
\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}



\newcommand{\bt}[1]{\begin{tabular}{#1}}
\newcommand{\et}{\end{tabular}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\ul}[1]{\underline{#1}}

%\newcommand{\eq}[1]{(\ref{#1})}

% macros
\def\g{\gamma}
\def\G{\Gamma}
% \def\a{\alpha}
% \def\g{\gamma}
% \def\S{\Sigma}
% \def\s{\sigma}
% \def\o{\omega}
% \def\l{\lambda}
% \def\d{\delta}
\def\N{\mathcal N}
\def\F{\mathcal F}
\def\L{\mathcal L}

\def\diag{\mbox{diag}}

\newcommand{\st}{\textrm{subject to}}
\DeclareMathOperator*{\mini}{minimise}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\trace}{tr}


%% Macros from Jakob Verbeek
\def\code#1{\begin{quote}{\tt #1}\end{quote}}
\def\I{{\rm I\!I}}                            % the indicator function
\def\R{{\rm I\!R}}                            % the real numbers
\def\matlab{\textsc{\small Matlab }}        % matlab add
%\def\Tr#1{\textrm{Tr}\{#1\}}                % trace
\def\diag#1{\textrm{diag}\left( #1 \right)} % diag
\def\Gauss#1#2#3{\mathcal{N}\left(#1 ; #2,#3\right)}   % Gaussian density
\def\ex#1#2{\textrm{I\!E}_{#1}\!\left[#2\right]}     % expectation
\def\half{\frac{1}{2}}              % half
\def\<{\langle}
\def\>{\rangle}

\def\nn{\nonumber}

% BOLD stuff
\def\alphabold{\mbox{\boldmath $\alpha$}}
\def\betabold{\mbox{\boldmath $\beta$}}
\def\gammabold{\mbox{\boldmath $\gamma$}}
\def\mubold{\mbox{\boldmath $\mu$}}
\def\kappabold{\mbox{\boldmath $\kappa$}}
\def\epsbold{\mbox{\boldmath $\epsilon$}}
\def\thetabold{\mbox{\boldmath $\theta$}}
\def\phibold{\mbox{\boldmath $\phi$}}
\def\Upsilonbold{\mbox{\boldmath $\Upsilon$}}
\def\eye{{\bf I}}



%\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45}
\newcommand{\hide}[1]{}
%\newcommand{\rar}{\rightarrow}
%\newcommand{\lar}{\leftarrow}
%\newcommand{\ol}{\overline}
%\newcommand{\Ra}{\Rightarrow}
%\newcommand{\upA}{\uparrow}
%\newcommand{\si}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\bfx}{{\bf x}}
\newcommand{\bfy}{{\bf y}}
\newcommand{\bfw}{{\bf w}}
\newcommand{\bfq}{{\bf q}}
\newcommand{\bfv}{{\bf v}}
\newcommand{\bfu}{{\bf u}}
\newcommand{\bfz}{{\bf z}}
\newcommand{\bfZ}{{\bf Z}}
\newcommand{\bfX}{{\bf X}}
\newcommand{\bfY}{{\bf Y}}
\newcommand{\bfV}{{\bf V}}
\newcommand{\bmu}{{\bm \mu}}
\newcommand{\bfW}{{\bf W}}
\newcommand{\bfP}{{\bf P}}
\newcommand{\bfQ}{{\bf Q}}
\newcommand{\bfS}{{\bf S}}
\newcommand{\bfA}{{\bf A}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bfb}{{\bf b}}
\newcommand{\bfd}{{\bf d}}
\newcommand{\bfD}{{\bf D}}

\newcommand{\tbf}{{\tilde{\bf f}}}
%\newcommand{\O}{{\Omega}}
\newcommand{\bfO}{{\bf \Omega}}
\newcommand{\bfG}{{\bf \Gamma}}


\newcommand{\bfh}{{\bf h}}
%\newcommand{\E}{\mathrm{E}}$
\newcommand{\V}{\mathrm{Var}}

\newcommand{\Cov}{\mathrm{Cov}}

%\newcommand{\bfxx}{[\begin{array}{l}{\tilde {\bf x}_n}\\{\tilde {\bf f}({\bf x}_n)\end{array}]}
%\newcommand{\bfwz}{[\begin{array}{l}{\bf w} \\ {\bf z}\end{array}]}

\newcommand{\al}{{\alpha}}
\DeclareMathOperator*{\E}{\mathbb{E}}
